Generalized quantum Zeno dynamics and ergodic means

We prove the existence of uniform limits for certain sequences of products of contractions and elements of a family of uniformly continuous propagators acting on a Hilbert or a Banach space. From the point of view of Quantum Physics, the considered sequences can represent the evolution of a system whose dynamics, described by a continuous propagator, is disturbed by a sequence of generic quantum operations (e.g., projective measurements or unitary pulses). This includes and also generalizes the so-called quantum Zeno dynamics. The time-evolution obtained from the limits of the considered sequences are described by propagators generated by ergodic means. The notion of such ergodic means is generalized in this paper to also include propagators of time-dependent generators, and thus our results can be used to develop new forms of active decoherence suppression. In a similar way, we also consider the effective time-evolution obtained from adding to the possibly time-dependent generator of the original propagator a generator of a uniformly continuous contraction semi-group with asymptotically increasing weight in the sum. By proving a generalized adiabatic theorem, it is shown that also for this set-up the resulting time-evolution is governed by a suitable ergodic mean.

==> intro.tex <==
Here, we study two questions motivated by some recent studies \cite{paz2012zeno,dominy2013analysis,bernad2017dynamical,burgarth2018generalized} appeared in the literature of quantum information processing aiming active decoherence avoidance.\par

Firstly, let $\hilbert$ be a Hilbert space and $\bhilbert$ be the space of bounded linear transformations of $\hilbert$ endowed with the usual sup-norm $\|\cdot\|$. Let $T\in\bhilbert$ be a contraction on $\hilbert$ and $K\in\bhilbert$ be the generator of $(F(t))_{t\geq 0}$, a uniformly continuous semi-group on $\hilbert$. We ask the question, what is the uniform limit and speed of convergence of the sequence
\begin{equation}
C_n\cdot \bigl(TF(t/n)\bigr)^n\qquad \qquad n\in\mathbb{N}_0\qquad\qquad t\in\mathbb{R}_0^+,
\label{Q1a}
\end{equation}
as $n$ tends to infinity, where the sequence $(C_n)_{n\in\mathbb{N}_0}\subset\bhilbert$ is a `natural' choice which guarantees an interesting, non-trivial limit in the uniform topology of $\bhilbert$. 

More generally, let $\banach$ be a Banach space, let $K:[t_{1},t_{2}]\rightarrow \bbanach$ be continuous on the finite, closed interval $[t_1,t_2]$. Define $F(\cdot,\cdot)$ as the solution of the initial value problem
\begin{eqnarray}
\partial_{1}F(u,v)&=&K(u)F(u,v)\qquad\qquad t_{1}\leq v\leq u\leq t_{2}\nonumber\\
F(v,v)&=&\mathbbm{1}_{\bbanach}.
\label{EQ1}
\end{eqnarray}
Assume that for each $n\in\N$, a partition $\mathfrak{T}_n$ of $[t_{1},t_{2}]$ defined through the sequences $t_{1}=t_{n,0}<t_{n,1}<\dots <t_{n,n}=t_{2}$ is given, such that the norms of these partitions converges to zero as $n$ tends to infinity. Then, the same question can be raised regarding the uniform limit of the products
\begin{equation}
C_n\cdot \prod_{l=0}^{n-1}TF(t_{n,l+1},t_{n,l})\qquad \qquad n\in\mathbb{N}_0
\label{Q1b}
\end{equation}
in $\bbanach$.
\par
Secondly, assume that $A\in\bhilbert$ generates a uniformly continuous contraction semi-group and let $K\in\bhilbert$. Then, if $\gamma>0$, we are interested in the large $\gamma$ behavior of the semi-group
\begin{equation}
F_\gamma(t)\vcentcolon=\exp\bigl((\gamma A+K)t\bigr)\qquad \qquad t\in\mathbb{R}_0^+.
\label{Q2}
\end{equation}

More generally, let $\banach$ be a Banach space, $A\in\bbanach$ be a generator of a uniformly continuous contraction semi-group and $K:[t_{1},t_{2}]\rightarrow \bbanach$ be continuous. Define $F_\gamma(\cdot,\cdot)$ as the solution of the initial value problem
\begin{eqnarray}
\partial_{1}F_\gamma(u,v)&=&\bigl(\gamma A+K(u)\bigr)F_\gamma(u,v)\qquad\qquad t_{1}\leq v\leq u\leq t_{2}\nonumber\\
F_\gamma(v,v)&=&\mathbbm{1}_{\bbanach}.
\label{Q2b}
\end{eqnarray}
Then, the same question can be raised regarding the large $\gamma$ behavior of (\ref{Q2b}).\par

%Our main results are the following theorems. \par
%\vspace{2mm}
%\noindent\textbf{Theorem 1.}
%\par
%\vspace{2mm}
%\noindent\textbf{Theorem 2.}




